The Next 700 ML-Enabled Compiler Optimizations

There is a growing interest in enhancing compiler optimizations with ML models, yet interactions between compilers and ML frameworks remain challenging. Some optimizations require tightly coupled models and compiler internals,raising issues with modularity, performance and framework independence. Practical deployment and transparency for the end-user are also important concerns. We propose ML-Compiler-Bridge to enable ML model development within a traditional Python framework while making end-to-end integration with an optimizing compiler possible and efficient. We evaluate it on both research and production use cases, for training and inference, over several optimization problems, multiple compilers and its versions, and gym infrastructures.

==> tables/tab-model-runner-characteristics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Characteristics of different model runners}
\label{tab:modelrunner-characteristics}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{c}{\textbf{}} & \textbf{gRPC} & \textbf{Pipes} & \textbf{ONNX} & \textbf{TF} \\
\midrule
\begin{tabular}[c]{@{}l@{}}Multithreaded \\ Compilation\end{tabular} & \xmark & \xmark & \cmark & \cmark \\[0.25cm]
\begin{tabular}[c]{@{}l@{}}Distributed\\ Training\end{tabular} & \cmark & \xmark & - & - \\[0.25cm] 
\begin{tabular}[c]{@{}l@{}}Need for separate\\ model process\end{tabular} & \cmark & \cmark & \xmark & \xmark \\[0.25cm]
Autoserialization & \cmark & \cmark & - & - \\[0.2cm]
\begin{tabular}[c]{@{}l@{}}ML Framework\\ agnostic\end{tabular} & \cmark & \cmark & \cmark & \xmark \\[0.25cm]
\begin{tabular}[c]{@{}l@{}}Additional code\\ by compiler writer\end{tabular} & $\uparrow$ & $\downarrow$ & $\uparrow$ & $\downarrow$ \\[0.25cm]
\begin{tabular}[c]{@{}l@{}}Serialization \\ Requirement\end{tabular} & $\uparrow$ & $\uparrow$ & - & - \\[0.25cm]
Time overhead & $\uparrow$ & $\uparrow$ & $\downarrow$ & $\downarrow$ \\
\begin{tabular}[c]{@{}l@{}}Communication\\ Errors\end{tabular} & Possible & Possible & Not possible & Not possible \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/tab-rel-works-comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[ht]
\centering
\caption{Different ML/RL requirements for previous works}
\label{tab:rel-works-comp}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllll}
\toprule
 & \multicolumn{1}{c}{\textbf{Communication}} & \multicolumn{1}{c}{\textbf{Model Input}} & \multicolumn{1}{c}{\textbf{Model Output}} & \multicolumn{1}{c}{\textbf{Commn Freq}} & \multicolumn{1}{c}{\textbf{\#Agents}} & \multicolumn{1}{c}{\textbf{Model Type}} & \multicolumn{1}{c}{\textbf{ML Framework}} \\
 \midrule
\textbf{SLP Vect (Mendis, NeurIPS'19)} & ?? & LLVM IR & Instructions to pack & ?? Once at the end? & Single Agent & GGNN & ?? \\
\textbf{NeuroVectorizer (CGO'20)} & pragmas in source & Code2Vec vectors & \begin{tabular}[c]{@{}l@{}}source code with pragma \\ added in Python\end{tabular} & None & Single Agent & FCNN & Keras, RLLib \\
\textbf{Reg Alloc - DD  (LLVM-HPC'20)} & No integration & Interference graph & Coloured IG & None & ML & LSTM & TensorFlow \\
\textbf{Reg Alloc - KIm (CGO'22)} & ?? & PBQP Graph & Allocated PBQP graph & Once, at the end ?? & Single Agent & GCN, ResNet & Pytorch \\
\textbf{POSET-RL (ISPASS'22)} & Opt Flags & IR2Vec vectors & Pass sequence & \begin{tabular}[c]{@{}l@{}}Multiple times \\ per episode\end{tabular} & Single Agent & FCNN & PyTorch, RLLib \\
\textbf{Loop Dist (LLVM HPC'22)} & Python Wrappers & IR2Vec vectors & DIst seq & Once, at the end & Two agents & GNN, FCNN & PyTorch, RLLib \\
\textbf{Inliner} & Precompiled TF model & Features & Yes/No & Once, at the end & Single Agent & FCNN & TensorFlow \\
\textbf{RL4ReAl (CC'23)} & gRPC & \begin{tabular}[c]{@{}l@{}}IG + node level \\ embeddings\end{tabular} & color map & \begin{tabular}[c]{@{}l@{}}Multiple times \\ per episode\end{tabular} & \begin{tabular}[c]{@{}l@{}}Four agents; \\ hierarchical\end{tabular} & GNN, FCNN & PyTorch, RLLib \\
\bottomrule
\end{tabular}%
}
\end{table*}
